A Nearly-Linear Time Algorithm for Linear Programs with Small Treewidth: A Multiscale Representation of Robust Central Path

Arising from structural graph theory, treewidth has become a focus of study in fixed-parameter tractable algorithms in various communities including combinatorics, integer-linear programming, and numerical analysis. Many NP-hard problems are known to be solvable in $\widetilde{O}(n \cdot 2^{O(\mathrm{tw})})$ time, where $\mathrm{tw}$ is the treewidth of the input graph. Analogously, many problems in P should be solvable in $\widetilde{O}(n \cdot \mathrm{tw}^{O(1)})$ time; however, due to the lack of appropriate tools, only a few such results are currently known. [Fom+18] conjectured this to hold as broadly as all linear programs; in our paper, we show this is true: Given a linear program of the form $\min_{Ax=b,\ell \leq x\leq u} c^{\top} x$, and a width-$\tau$ tree decomposition of a graph $G_A$ related to $A$, we show how to solve it in time $$\widetilde{O}(n \cdot \tau^2 \log (1/\varepsilon)),$$ where $n$ is the number of variables and $\varepsilon$ is the relative accuracy. Combined with recent techniques in vertex-capacitated flow [BGS21], this leads to an algorithm with $\widetilde{O}(n^{1+o(1)} \cdot \mathrm{tw}^2 \log (1/\varepsilon))$ run-time. Besides being the first of its kind, our algorithm has run-time nearly matching the fastest run-time for solving the sub-problem $Ax=b$ (under the assumption that no fast matrix multiplication is used). We obtain these results by combining recent techniques in interior-point methods (IPMs), sketching, and a novel representation of the solution under a multiscale basis similar to the wavelet basis.

==> edge-separator.tex <==
\subsection{Approximating a Balanced Separator} \label{subsec:apx_balance}

We present two approaches to \textsc{approxBalancedSeparator} as required by \cref{alg:make-elim-tree} when a tree decomposition is not given. The first directly invokes a result of Brandt and Wattenhofer.

\begin{theorem}[\cite{brandt2017approximating}]
	Let $G = (V,E)$ be a graph on $n$ vertices and $m$ edges. If $G$ contains an $\alpha$-separator of size $\tau$, then there exists a Las Vegas algorithm which finds an $(\alpha + \eps)$-separator of size $O( \eps^{-1} \tau^2 \log^{1+o(1)} n)$ in time $O(\eps^{-1} \tau^3 m \log^{2+o(1)}n)$ w.h.p..
\end{theorem}

Applied in our setting, we have:
\begin{theorem}
	Let $G = (V,E)$ be a graph on $n$ vertices and $m \leq n\tau$ edges. If $G$ contains an $1/2$-separator of size $\tau$, then there exists a Las Vegas algorithm which finds an $3/4$-separator of size $\widetilde{O}(\tau^2)$ in time $\widetilde{O} (n \tau^4)$ w.h.p..
\end{theorem}

\begin{comment}
\subsubsection{SDP Pseudo-approximation}

The second approach is based on the directed balanced edge separator algorithm of Arora and Kale~\cite{arora2016combinatorial}. %TODO: cite
It interestingly gives rise to a run-time dependent on the max-flow on an auxiliary graph.

\begin{theorem}\label{thm:sdp-edge-separator}
	Let $G = (V,E)$ be a graph with $n$ vertices, $m$ edges, and treewidth $\tau$. Suppose $S$ is an minimum $1/2$-vertex separator of $G$. Then we can compute a $\alpha$-balanced vertex separator $S'$ for some universal constant $\alpha$, such that $|S'| \leq O(\log n) |S|$. The algorithm runs in $\widetilde{O}(T_{maxflow})$ time, where $T_{maxflow} \leq O(m+n^{1.5})$ is the time it takes to compute a max-flow of an auxiliary graph with $O(n)$ vertices, $O(m)$ edges, and treewidth $O(\tau)$.
\end{theorem}
	
To begin, %, note that by Lemma~\ref{lem:tw-edge-bound}, $|E| \leq n\tau$.
we use a standard technique~\cite{leighton1999multicommodity} to reduce \textsc{undirected balanced vertex separator} to \textsc{directed balanced edge separator}:

An $1/2$-vertex separator in $G$ is represented by $(A,S,B)$, where $A \cup S \cup B = V(G)$, and $S$ is the vertex separator that disconnects vertices between $A$ and $B$, where $|A|,|B| \leq 1/2 |V(G)|$.  

Given a graph $G$ on $n$ vertices with treewidth $\tau$, we construct a weighted, directed graph $G'$,
where $V(G') = V(G) \cup \{v' :  v \in V(G)\}$, and $E(G') = \{(v,v') : v \in V(G)\} \cup \{(u',v) : (u,v) \in E(G)\} \cup \{(v',u) : (u,v) \in E(G)\}$. Note that $|V(G')| = 2n$ and $|E(G')| = O(m)$. We use $w$ to denote the edge capacities (or, for convenience, weights), and assign $w(v,v') = 1$ for all $v \in V(G)$, and $w(u,v) = +\infty$ for all other edges (equivalently, we may set this as $n$).

For any set $S \subseteq V(G)$, define the notation $S' = \{ v \;:\; v \in T\} \subseteq V(G')$. 

For a cut $(S, \bar{S})$ in $G'$, define $w(E(S, \bar{S}))$ to be the total weight of the edges going from $S$ to $\bar{S}$. For any $\alpha > 1/2$, the cut is $\alpha$-balanced if $|S|,|\bar{S}| \leq \alpha |V(G')|$. 
The minimum $\alpha$-edge separator is the $\alpha$-balanced cut $(S, \bar{S})$ that minimizes $w(E(S, \bar{S}))$. 

Due to the $+\infty$ weights, any minimum $\alpha$-edge separator $(S,\bar{S})$ in $G'$ only contains edges of the form $(v,v')$ for $v \in G$. Then the set $\widetilde{S} = \{ v \in G \;:\; (v,v') \in E(S,\bar{S})\}$ is an $\alpha$-vertex separator in $G$: 
Indeed, let $A = \{ v \in G \;:\; v \in S \setminus \widetilde{S}\}$ and $B = \{ v \in G \;:\; v \in \bar{S} \setminus \widetilde{S}\}$. There are no edges between $A$ and $B$ in $G$: Suppose for a contradiction there is $u \in A$ and $w \in B$. Since $(u,u') \notin (S, \bar{S})$, we know $u' \in A$, and similarly $w' \in B$. Then there would be directed edges $(u', w)$ and $(w', u)$ in $G'$, both with infinite capacity, in the cut $(S, \bar{S})$, giving the desired contradiction.
Since $|S|, |\bar{S}| \leq \alpha \cdot 2n$, we have $|A| = 1/2(|S| - |\widetilde{S}|) \leq \alpha \cdot n$, and similarly for $B$.

Conversely, any minimum $\alpha$-vertex separator $(A,S,B)$ in $G$ gives a $\alpha$-edge separator in $G'$ with the same size: Indeed, let $\widetilde{A} = A \cup A' \cup S$ and $\widetilde{B} = B \cup B' \cup S'$, then $(\widetilde{A}, \widetilde{B})$ is a cut in $G'$, with $E(\widetilde{A}, \widetilde{B}) = \{ (v,v') \;:\; v \in S\}$. To see this cut is $\alpha$-balanced, note that $|\widetilde{A}| = 2|A| + |S| \leq 2 \alpha n + (1-\alpha)n = (1+\alpha)n = \frac{1+\alpha}{2} \cdot (2n) < \alpha \cdot |V(G')|$, and similarly for $|\widetilde{B}|$.

If we view $G'$ as an undirected graph (by ignoring the edge orientations), then its treewidth is at most double the treewidth of $G$ by construction.

Now, we use the techniques from~\cite{arora2016combinatorial} to compute a balanced cut in $G'$. First, we define a $t$ pseudo-approximation to be an $\alpha$-balanced cut for some universal constant $\alpha$, whose size is within a factor $t$ of the optimal $1/2$-balanced cut. The~\cite{arora2016combinatorial} algorithm maintains a guess $\tau'$ of the minimum separator size in $G'$, determined by the doubling-trick to binary search for it, at each iteration running the optimization algorithm. We may assume it is $\widetilde{O}(\tau)$. 

%Let $\tau$ be the algorithm's guess of the minimum separator size; in the discussion below we may assume it is $\widetilde{O}(\tw(A))$. This is . Either we find a primal-feasible solution with value $< \tau$, at which point we re-run the algorithm with a new guess, or we find a dual-feasible solution of value $(1-\delta)\tau$ for some arbitrarily small $\delta$.

\begin{theorem} [\cite{arora2016combinatorial}, Lemma 3, Theorem 7]
	Let $L,R \subseteq V(G)$, and define the auxillary graph $G_{L,R}''$ to be $G'$ with additional source and sink nodes $s,t$, directed edges from $s$ to each vertex in $L$, and from each vertex in $R$ to $t$, with capacities $O(\log n \cdot \tau'/n)$. Suppose we can compute the directed max flow in $G''$ in time $O(T_{maxflow})$, then there is an $O(\log n)$ pseudo-approximation algorithm to the minimum $1/2$-edge separator that takes $\widetilde{O}(T_{maxflow})$ time, consisting of using $\polylog n$ max-flow computations on auxilliary graphs $G_{L,R}''$ for different sets $L,R$. 
\end{theorem}

Observe that $G''$ is obtained from $G'$ by adding two new vertices, and therefore $\tw(G'') = O(\tw(G))$.

We leave the following conjecture:
\begin{conjecture}
	A max flow in $G''$ can be computed in time $\widetilde{O}(n\tau^2)$. 
\end{conjecture}
\begin{lemma}[\cite{arora2016combinatorial}, Lemma 3]
	Let $S \subseteq V$ be a set of vertices of size $\Omega(n)$. Suppose we are given, for all $i \in S$, vectors $\mathbf{v}_i, \mathbf{w_i}$ of length $O(1)$, such that $\sum_{i, j \in S} \norm{\mathbf{v}_i - \mathbf{v}_j}^2 \geq \Omega(n^2)$, and for all $i,j$, $\norm{\mathbf{w}_i - \mathbf{w}_j}^2 \leq o(1)$. Define the directed distance $d(i,j) = \norm{v_i - v_j}^2 - \norm{w_i - v_i}^2 + \norm{w_j - v_j}^2$. For any given value $\tau$,
	there is an algorithm which, using a single max-flow computation, either outputs a valid $O(\frac{\log n \cdot \tau}{n})$-regular directed flow $f_p$ such that $\sum_{ij} f_{ij} d(i,j) \geq \tau$, or an $\alpha'$-balanced cut of expansion $O(\log n \cdot \tau/n)$.
\end{lemma}
\end{comment}

%The algorithm identifies disjoint vertex sets $L, R \subseteq V(G')$, and creates the auxiliary graph $G''$ by adding source and sink nodes $s,t$ and connecting them to $L$ and $R$ respectively, with capacity $O(\log(n) \tau/n)$ on each additional edge, and computes the max flow on $G''$. Any flow on $G''$ will be a $d := O(\log(n) \tau/n)$-regular flow on $G'$ (meaning the flow from every vertex is bounded by $d$). For a vertice $v \in L$, since the capacity of the edge from $s$ to $v$ is $d$, we know the flow out from $L$ is at most $d$. If the total flow has value less than $(\alpha/2) \cdot \beta \log n \cdot \tau$, then the corresponding min cut will be $\alpha/2$-balanced.


\begin{comment}
The algorithm is an SDP version of multiplicative weights; it begins with an SDP formulation of {\sc Balanced Edge Separator} and its dual. 
At iteration $i$, we have a candidate primal solution $\mathbf{X}^{(i)}$. It then calls {\sc Oracle}, which answers either with a matrix $\mathbf{F}^{(i)}$ and a vector $\mathbf{y}^{(i)}$, that is used to update $\mathbf{X}^{(i)}$, or a $\alpha'$-balanced cut of size $O(\log n \cdot \tau)$. The run-time analysis is as follows:

\begin{theorem}[\cite{arora2016combinatorial}, Theorem 3]\label{thm:arora-runtime}
	In the primal-dual SDP algorithm, assuming {\sc Oracle} returns feedback matrices for $T = \frac{8\rho^2 R^2 \log n}{\delta^2 \tau^2}$ iterations, then we can produce a feasible dual solution with objective value at least $(1-\delta)\tau$.
\end{theorem}

Here, $\rho$ is the width parameter of the {\sc Oracle}, which is the smallest non-negative value such that for every primal candidate $\mathbf{X}$, {\sc Oracle} returns a feedback matrix $\mathbf{F}$ and dual vector $\mathbf{y}$ satisfying $\norm{\mathbf{F}} \leq \rho$. %TODO: (actually this is a bound on the dual conditions. more later). %TODO
$R$ is a bound on the trace of the solution, that is, $Tr(\mathbf{X}) \leq R$. We may assume without loss of generality that the first constraint is $\mathbf{X} \bullet \mathbf{I} := Tr(\mathbf{X} \cdot \mathbf{I}) \leq b_1 = R$.

The {\sc Oracle} uses of the following lemma, which either helps the algorithm to make progress at an iteration, or already returns a suitable solution. The conditions of the lemma are guaranteed by the algorithm.
\begin{lemma}
	Let $S \subseteq V$ be a set of vertices of size $\Omega(n)$. Suppose we are given, for all $i \in S$, vectors $\mathbf{v}_i$ of length $O(1)$, such that $\sum_{i, j \in S} \norm{\mathbf{v}_i - \mathbf{v}_j}^2 \geq \Omega(n^2)$, and a quantity $\tau$. 
	Then there is an algorithm which, using a single max-flow computation, either outputs a valid $O(\frac{\log n \cdot \tau}{n})$-regular flow $f_p$ such that $\sum_{ij} f_{ij} \norm{\mathbf{v}_i - \mathbf{v}_j}^2 \geq \tau$, or an $\alpha'$-balanced cut of expansion $O(\log n \cdot \tau/n)$.
\end{lemma}
\end{comment}
%Using $\rho = O(\log n \cdot \tau/n)$ and $R = n$ in Theorem~\ref{thm:arora-runtime}, we get the overall result of Theorem~\ref{thm:sdp-edge-separator}.

==> initial-point.tex <==
\section{Robust Interior Point Algorithm for General Convex Sets\label{sec:Robust-IPM}}

In this section, we give a robust interior point method for the optimization
problem 
\begin{equation} \tag{CP}
\min_{Ax=b,x_{i}\in K_{i}\text{ for }i\in[m]}c^{\top}x\label{eq:problem}
\end{equation}
where $A$ is a $d \times n$ matrix, $x_{i}\in K_{i}\subset\R^{n_{i}}$, and $x$ is the concatenation
of $x_{i}$ lying inside the domain $K\defeq\prod_{i=1}^{m}K_{i}\subset\R^{n}$
with $n=\sum_{i=1}^{m}n_{i}$.  The main result of this section is the following:
\begin{restatable}{theorem}{thmIPMframework}\label{thm:IPM_framework}
Consider the convex program \cref{eq:problem}. Given $\nu_{i}$-self-concordant barriers $\phi_{i}:K_{i}\rightarrow\R$ with its minimum $x_i$. Assume that
	\begin{enumerate}
		\item Lipschitz constant of the program: $\norm{c}_2 \leq L$.
		\item Diameter of the polytope: For any $x \in \prod_{i=1}^m K_i$, we have $\norm{x}_2 \leq R$.
	\end{enumerate}
Let $w \in \R_{\geq 1}^m$ be any weight vector, and $\kappa=\sum_{i=1}^{m}w_{i}\nu_{i}$. For any $0 < \eps \leq 1$, \cref{alg:IPM_framework} outputs an approximate solution $x$ in $O(\sqrt{\kappa}\log(\kappa/\eps))$ steps, such that
			\begin{align*}
				c^\T x &\leq \min_{Ax = b, \; x \in \prod_{i=1}^m K_i} c^\T x + LR \cdot \eps \\
				\norm{Ax - b}_2 &\leq \eps \cdot (R \norm{A}_2 + \norm{b}_2) \\
				x &\in \prod_{i=1}^m K_i.
			\end{align*}
\end{restatable}

\begin{rem}\label{rem:IPM-universal-barrier}
If the barrier functions $\phi_i$ is not given, we can use $w_i = 1$ and universal barrier functions $\phi_i$ for $K_i$. In this case, the algorithm takes $O(\sqrt{n}\log(\kappa/\eps))$ steps, and the cost of computing a good enough approximation of $\nabla \phi_i$ and $\nabla^2 \phi_i$ both takes $n_i^{O(1)} \log(m M)^{O(1)}$ time for each $i$, assuming the following mild conditions:
	\begin{enumerate}
		\item We can check if $x_i$ is in $K_i$ in time  $n_i^{O(1)}$.
		\item $B(x_i,r_i) \subset K_i \subset B(x_i, M r_i)$ for some given $x_i$ and $r_i$. %TODO: Q: is this x_i the same as the minimizer x_i of phi_i?
	\end{enumerate}
\end{rem}

Our algorithm and the proof is similar to \cite{DBLP:conf/colt/LeeSZ19}, the main difference being that we do not use an approximate $t$ in the formula, which is needed for our main data
structure. Therefore, we include the proof for completeness. To slightly
simplify the proof and the algorithm for the data structure, we used the potential $\cosh(\|\cdots\|)$ instead
of $\exp(\|\cdots\|)$ as in \cite{DBLP:conf/colt/LeeSZ19} because the new one is differentiable
at $\|\cdots\|=0$.

Although we will simply use $w_i = 1$ for all $i$ in this paper,
we support the use of other weights in case it is useful in the future.
Another improvement over \cite{DBLP:conf/colt/LeeSZ19} is that our bound is tight even for the case some $\nu_{i}$ is much larger than other $\nu_{i}$. We note that it is an interesting open question to extend it to dynamic weighted barriers such as the Lee-Sidford
barrier \cite{DBLP:journals/corr/abs-1910-08033} (beyond the case $n_{i}=1$).

\subsection{Overview}

Our algorithm is based on interior point methods which follow some
path $x(t)$ inside the interior of the domain $K$. The path
starts at some interior point of the domain $x(1)$ and ends at the
solution $x(0)$ we want to find. One commonly used path is defined
by 
\begin{equation}
x(t)=\arg\min_{Ax=b}c^{\top}x+t\sum_{i=1}^{m}w_{i}\phi_{i}(x_{i})\label{eq:ipm_formula}
\end{equation}
where $\phi_{i}$ are self-concordant barrier functions on $K_{i}$.
The weights $w\in\R_{>0}^{m}$ are fixed throughout the algorithm.
\begin{definition}[\cite{Nesterov1998}]\label{defn:self-concordant}
A function $\phi$ is a $\nu$-self-concordant barrier for a non-empty
open convex set $K$ if $\dom\phi=K$, $\phi(x)\rightarrow+\infty$
as $x\rightarrow\partial K$, and for any $x\in K$ and for any $u\in\R^{n}$
\[
D^{3}\phi(x)[u,u,u]\leq 2 \|u \|_{\nabla^2 \phi(x)} \text{ and }\|\nabla\phi(x)\|_{(\nabla^2 \phi(x))^{-1}}\leq\sqrt{\nu}.
\]
A function $\phi$ is a self-concordant barrier
if the first condition holds.
\end{definition}

For many convex sets, we have
an explicit barrier with $\nu=O(n)$. For the case of linear programs, the convex set $K_i = [\ell_i,u_i]$ and one can use the log barrier $-\log(u_i - x) - \log(x - \ell_i)$. It has self-concordance $1$. Throughout this section, we only use the fact that $\nu\geq1$ to simplify formulas.
\begin{lemma}[{\cite[Corollary 4.3.1]{Nesterov1998}}]
The self-concordance $\nu$ is larger than $1$ for any barrier function.
\end{lemma}

Since $\phi_{i}$ blows up on $\partial K_{i}$, $x(t)$ lies in the
interior of the domain for $t>0$ (if the interior is non-empty).
By the definition of $x(t)$, $x(0)$ is a minimizer of the problem
\cref{eq:problem}. In \cref{sec:initial-point-reduction}, we
show how to find the initial point $x(1)$ quickly by reformulating
the problem into an equivalent form. In \cref{sec:IPMAlgo} to \cref{subsec:GD_on_Phi}, we explain how to follow the path from $x(1)$ to $x(0)$. We prove the correctness in the rest of the subsections.


\subsection{Initial Point Reduction}\label{sec:initial-point-reduction}

To generate an initial feasible point for the central path, we follow the reduction from~\cite{DBLP:conf/colt/LeeSZ19}.

\begin{lemma}\label{lem:initial-point-reduction}
	Given a convex program \cref{eq:problem}, suppose for each $i \in [m]$, we are given a $\nu_i$-self concordant barrier function $\phi_i$ for $K_i$, and $x^{(0)} = \argmin_x \sum \phi_i(x_i)$, where $x_i \in K_i$. Assume that
	\begin{enumerate}
		\item Diameter of the polytope: For any $x \in \prod_{i=1}^m K_i$, we have $\norm{x}_2 \leq R$.
		\item Lipschitz constant of the program: $\norm{c}_2 \leq L$.
	\end{enumerate}
	Then, for any $0 < \eps \leq 1$, the modified convex program 
	\begin{align}\label{eqn:ERM-program} 
	\min \quad &\bar{c}^\T \bar{x}  \tag{$\overline{CP}$}  \\
	s.t. \qquad \bar{A} \bar{x} = \bar{b},  &\quad
	\bar{x} \in \prod_{i=1}^m K_i \times \mathbb{R}_+^d \nonumber
	\end{align} 
	with
	\[
	\bar{A} = [	A \;|\; D(b- Ax^{(0)})], \;
	\bar{b} =  b \; \text{and } 
	\bar{c} = \begin{bmatrix}
	\frac{\eps}{LR} \cdot c \\ \frac{1}{d}\mathbf{1}
	\end{bmatrix}
	\]
	where $D(b-Ax^{(0)})$ is the diagonal matrix with $b-Ax^{(0)}$ on the diagonal,
	satisfies the following:
	\begin{enumerate}
		\item $\bar{x} = \begin{bmatrix}
			x^{(0)} \\ \mathbf{1}
		\end{bmatrix}$ and
		$\bar{y} = \mathbf{0}_d$ are feasible primal and dual vectors, with slack
		$\bar{s} = \begin{bmatrix}
		\frac{\eps}{LR} \cdot c \\ \mathbf{1}
		\end{bmatrix}$, and
		$\norm{\bar{s} + \grad \bar{\phi} (\bar{x})}_{\bar{x}}^* \leq \eps$, where $\bar{\phi} (\bar{x}) = \sum_{i=1}^m \phi_i (\bar{x}_i) - \sum_{i=m+1}^{m+d} \log (\bar{x}_{i})$.
		\item For any $\bar{x}$ such that $\bar{A} \bar{x} = \bar{b}$, $\bar{x} \in \prod_{i=1}^m K_i \times \mathbb{R}_+$, and $\bar{c}^\T \bar{x} \leq \overline{OPT} + \frac{\eps^2}{10 n^4}$, the vector $\bar{x}_{1:n}$ is an approximate solution to the original convex program $(CP)$ in the following sense:
			\begin{align*}
				c^\T \bar{x}_{1:n} &\leq \min_{Ax = b, \; x \in \prod_{i=1}^m K_i} c^\T x + LR \cdot \eps \\
				\norm{A\bar{x}_{1:n} - b}_2 &\leq \eps \cdot (R \norm{A}_2 + \norm{b}_2) \\
				\bar{x}_{1:n} &\in \prod_{i=1}^m K_i.
			\end{align*}
	\end{enumerate}
\end{lemma}

The proof follows directly from Lemma D.2 of~\cite{DBLP:conf/colt/LeeSZ19}, with the exception that  they have one additional variable $x_{m+1}$ in $\bar{x}$ and a dense column $b-Ax^{(0)}$ concatenated to $A$, whereas we have $d$ additional variables $x_{m+1},\dots, x_{m+d}$ in $\bar{x}$, and correspondingly the diagonal matrix $D(b-Ax^{(0)})$. 
\begin{comment}
Strictly speaking, this alteration of ~\cite{DBLP:conf/colt/LeeSZ19} is valid only if we have the constraints $x_i=x_j$ for pairwise $i,j \in \{n+1,\dots, n+d\}$. However, we note that as the interior point method converges, we must have $x_{n+1},\dots, x_{n+d} \to 0$, and so the equality constraints are satisfied implicitly.
\end{comment}

Finally, observe that $\tw(A) = \tw(\bar{A})$, since concatenating a diagonal matrix to $A$ does not change the adjacency relations in the graph. 

\begin{comment}
In the above reduction, note that $tw(\bar{A})$ can become much greater than $tw(A)$, depending on the non-zero pattern of the additional column $b-Ax^{(0)}$ in $\bar{A}$. We make a further reduction and leverage Theorem~\ref{thm:initial-point-reduction} resolve this.

\begin{theorem}\label{thm:initial-point}
	Let $A,b,c,\bar{A}, \bar{b}, \bar{c}, x^{(0)}$ be defined as in Theorem~\ref{thm:initial-point-reduction}. Given the elimination tree $T$ for $A$, we can construct a modified convex program
	\begin{equation*}\tag{$CP'$}
	\min \; c'^\T \begin{bmatrix}	x \\ y \end{bmatrix}
	 \quad \text{s.t.}  \quad A' 
	\begin{bmatrix}	x \\ y \end{bmatrix}  = b', 
	\quad x \in \prod_{i=1}^m K_i, \quad  y \in \mathbb{R}_+^{d'},
	\end{equation*} 
	based on $T$, where $A' \in \mathbb{R}^{O(d) \times (n+d')}$ and $d' = O(d)$, such that
	%TODO: update this notation
	\begin{enumerate}
		\item 
		$x' = \begin{bmatrix}
		x^{(0)} \\ \frac{1}{d'} \mathbf{1}
		\end{bmatrix}$ and $\mathbf{0}$ 
		are feasible primal and dual vectors with slack
		$s' = \begin{bmatrix}
		\frac{\eps}{LR} \cdot c \\ \frac{1}{d'} \mathbf{1} \end{bmatrix}$, and
		$\norm{s' + \grad \bar{\phi} (x')}_{x'}^* \leq \eps$, %TODO: update this notation
		where $\bar{\phi} (x') = \sum_{i=1}^m \phi_i (x'_i) - \sum_{j} \log (y_j)$.
		\item For any $(x,y) \in \prod_{i=1}^m K_i \times \mathbb{R}_+^{d'}$ such that $A' [x \; y]^\T = b'$, and ${c'}^\T [x \; y]^\T \leq OPT' + \eps^2$, the vector $x$ is an approximate solution to the original convex program $(CP)$ in the following sense:
		\begin{align*}
		c^\T x &\leq \min_{Ax = b, \; x \in \prod_{i=1}^m K_i} c^\T x + LR \cdot \eps \\
		\norm{Ax}_1 &\leq 3\eps \cdot (R \norm{A}_1 + \norm{b}_1) \\
		x &\in \prod_{i=1}^m K_i.
		\end{align*}
		\item We can construct an elimination order and tree $T'$ for $A'$, such that $height(T') \leq O(height(T) \cdot \log d)$. Furthermore, if $t_v$ is the height of vertex $v$ in $T$, and $t_i'$ is the height of vertex $i$ in $T'$, then 
		\[\sum_{v \in V(T')} t_v'^2 \leq O(\log d \cdot \sum_{v \in V(T)} t_v^2).\]
		\item Each column of $A'$ has at most $tw(A)$ non-zero entries.
	\end{enumerate}
	%TODO: time it takes?
\end{theorem}

\begin{proof}
	Let $(CP')$ denote the convex program we construct, with constraint matrix $A' [x \; y]^\T = b'$. There will be a natural correspondence between the rows of $A$ and the first $d$ rows of $A'$. In the construction, $y$ are new variables; we index the entries of $y$ by some $S \subset [d]$ rather than integers.
		
	\subsection{Algorithm}
	Let $G$ denote the support graph of $A$, where $V(G) = V(T) = \{v_1, \dots, v_d\}$, and $v_i$ is the $i$-th constraint of $Ax = b$. We may assume without loss of generality that $T$ is connected.
	
	Crucially, $A'$ will rely on the structure of $T$, so that we can bound the resulting height of $T'$. First, we give the algorithmic construction of $A'$. We use matrix notation and linear equations interchangeably.
	
	\begin{algorithm}[H]\caption{Construct $LP'$ with feasible initial point} \label{alg:dense-col-mod}
		\begin{algorithmic}[1]
			\State $A'\leftarrow [A \;|\; D(b - A x^{(0)}) ]$
			\Comment $D(v)$ is a diagonal matrix with $v$ on the diagonal
			\State $b' \leftarrow \bar{b}$
			\ForEach{$v_i \in V(T)$ with $k>1$ children $v_{i_1}, v_{i_2}, \dots, v_{i_k}$}
				\State \text{add constraints (translates to adding rows to $A'$ and entries to $b'$)} 
					\begin{align*}
					y_{\{i_1\}} &= y_{\{i_1, i_2\}} \\
					 y_{\{i_2\}} &= y_{\{i_1, i_2\}} \\
					 &\;\vdots \\
					 y_{\{i_{k-1}\}} &= y_{\{i_{k-1}, i_k\}}\\
					 y_{\{i_k\}} &= y_{\{i_{k-1}, i_k\}} \\
					 y_{\{i_1,i_2\}} &= y_{\{i_1,i_2, i_3,i_4\}} \\
					 y_{\{i_3,i_4\}} &= y_{\{i_1,i_2, i_3,i_4\}} \\
					 &\;\vdots \\
					 y_{\{i_1, \dots, i_{k/2}\}} &= y_{\{i_1,\dots, i_k\}} \\
					 y_{\{i_{k/2+1}, \dots, i_k\}} &= y_{\{i_1, \dots, i_k\}} \\
					 y_{\{i_1, \dots, i_k\}} &= y_{\{i\}} 
			 		\end{align*}
			\EndFor
			\State $c' \leftarrow \begin{bmatrix}
			\frac{\eps}{LR}\cdot c \\ \frac{1}{d'} \cdot \mathbf{1}
			\end{bmatrix}$ 
			\Comment $\frac{1}{d'} \cdot \mathbf{1}$ is the constant vector of length $d'$, where $d'$ is the number of new variables
		\end{algorithmic}
	\end{algorithm}
	
	\subsection{Algorithm Explanation}
	We construct $A'[x\;y]^\T=b'$ to be an extension of $\bar{A}\bar{x} = \bar{b}$. 
	
	In lines 1-3, we concatenate $A$ with an $d \times d$ diagonal matrix $D(b-Ax^{(0)})$ (rather than the column $b-Ax^{(0)}$ for $\bar{A}$). We use $y_{\{1\}}, \dots, y_{\{d\}} \in \mathbb{R}_+$ to denote the new variables introduced. Compared against $\bar{A} \bar{x} = \bar{b}$, we see that\\
	$\begin{bmatrix}
		A \;|\;b-Ax^{(0)} 
	\end{bmatrix}	
	\begin{bmatrix} x \\ x_{n+1}\end{bmatrix}
	= \bar{b}
	$ becomes
	$\begin{bmatrix}
		A \;|\; D(b-Ax^{(0)}) 
	\end{bmatrix}
	\begin{bmatrix}x \\ y_{\{1\}} \\ \vdots \\ y_{\{d\}} \end{bmatrix}
	 = b'$, where $x \in \mathbb{R}^{n}$.
	 
	 A solution here might not yield a solution to the original $\bar{A}\bar{x} = \bar{b}$. To ensure that it does, we need to add constraints and intermediate variables to ensure $y_{\{1\}} = \dots = y_{\{d\}}$, after which we can set $\bar{x}_{n+1}$ as that value, and $\bar{x}_i = x_i$ for all other $i$. How these constraints are added will affect the resulting elimination tree. 
	 
	 Lines 4-6 iterates through each vertex in $T$, and adds new constraints based on the arrangement of its children. 
	
	\subsection{Correctness}
	First, observe that $OPT' = \overline{OPT}$ where the two are optimal values for $(CP')$ and $(\overline{CP})$ respectively.
	
	Second, any $(x,y) \in \prod_{i=1}^m K_i \times \mathbb{R}_+^{d'}$ satisfying $A' [x \; y]^\T =b'$ also satisfies $y_S = y_T$ for all valid indices $S,T \subseteq [d]$; hence, $\bar{A}[x \; y_{\{1\}}]^\T=\bar{b}$. If on top of this, we also have $c'^\T [x \; y]^\T \leq OPT' + \eps^2$, then $(x, y_{\{1\}}) \in \prod_{i=1}^m K_i \times \mathbb{R}_+$ satisfies $\bar{A} [x \; y_{\{1\}}]^\T = \bar{b}$, and $\bar{c}^\T [x \; y_{\{1\}}]^\T \leq \overline{OPT} + \eps^2$. Then by Theorem~\ref{thm:initial-point-reduction}, $x$ satisfies part (2) in the theorem statement.
	
	Each column of $A$ has at most $tw(A)$ non-zero entries, by definition of tree-width. In our modification, we note that the first $n$ columns of $A'$ are simply those of $A$ padded with zeros; the additional columns each has a constant number of non-zero entries, since each $y_S$ exists in a constant number of new constraints. Hence part (4) is satisfied.
	
	It is easy to check that part (1) is satisfied as well by relating it Theorem~\ref{thm:initial-point-reduction}.
	
	The dimension of $A'$ is as follows: At the vertex $v \in V(T)$ with $k$ children, the construction introduces $O(k)$ new variables of the form $y_S$. Hence, we introduce $d' = O(d)$ new variables in total. Furthermore, since each $y_S$ appears in at most 3 constraints, there are $O(d)$ total new constraints. Therefore, $A' \in \mathbb{R}^{O(d) \times (n+d')}$.
	
	It remains to examine the elimination tree for $A'$.
	\subsection{Change from $G$ to $G'$, and from $T$ to $T'$}
	
	Recall $V(G) = V(T) = \{v_1,\dots, v_d\}$, where vertex $v_i$ corresponds to the $i$-th row of $A$. Let $G'$ denote the support graph of $A'$. Let $p_T(v_i)$ denote the parent of $v_i$ in $T$. 
	
	The first $d$ rows of $A'$ is given by $[A \; | \; D(b-Ax^{(0)})]$; we label the corresponding vertices in $G'$ by $\{v_1, \dots, v_d\}$ in order. Then, note that $G'[\{v_1, \dots, v_d\}] \cong G$, since the concatenated diagonal matrix does not contribute any new edges.
	
	The new constraints added in Algorithm~\ref{alg:dense-col-mod} correspond to additional vertices in $G'$. We label such a constraint (vertex) by a subset $S$ where $S \subset [d]$ as follows: constraint $S$ is the unique constraint of the form $y_S = y_R$, where $R$ is a subset containing $S$. For example, in Figure~\ref{fig:G-to-Gp}, vertex $v_{\{3,4\}}$ is the constraint $y_{\{3,4\}} = y_{\{1,2,3,4\}}$. 
	
	In iteration $v_i$ of lines 4-6 of Algorithm~\ref{alg:dense-col-mod}, we modify vertex $v_i$ with children $v_{i_1}, \dots, v_{i_k}$. The support graph changes as follows: new vertices $v_{\{i_1\}}, \dots, v_{\{i_k\}}, v_{\{i_1,i_2\}}, \dots, v_{\{i_1, \dots, i_{k}\}}, v_{\{i\}}$ are added to $G'$ (if they haven't been added already). Each new vertex $v_{\{i_j\}}$ is connected to $v_{i_j}$, since constraints $\{i_j\}$ and $i_j$ share the variables $y_{\{i_j\}}$. A pair of new constraints $y_S = y_R$ (labelled by $S$) and $y_R = y_U$ (labelled by $R$), where $S,R,U \subseteq \{i_1, \dots, i_k\}$, adds the edge $v_S v_R$, since constraints $S$ and $R$ share the variable $y_R$. For $S = \{i_1,\dots,i_k\}$, constraint $S$ shares the variable $y_{\{i\}}$ with constraints $i$ and $\{i\}$, adding the edge $v_S v_i$ and $v_S v_{\{i\}}$. One straightforward observation of this construction is that for any vertex $v_S$ with $S \subseteq [d]$, if $i,j \in S$, then $p_T(v_i) = p_T(v_j)$.
	
	We illustrate this change to the support graph and elimination tree with the following example, which corresponds to one iteration of the loop in Algorithm~\ref{alg:dense-col-mod}, for the vertex $v_8$ with children $v_1, v_2,\dots, v_7$ in $T$.
	
	\begin{figure}[H]
		\centering 
		\includegraphics[scale=0.9]{fig-T-node}
		\caption{The elimination tree $T$ at a single vertex, with seven children. For simplicity, we label a vertex $v_i$ by its subscript $i$.}
		\label{fig:ex-elim-tree-old}
	\end{figure}

	After new constraints are added in the current iteration, $G'$ locally looks like the following:
	\begin{figure}[H]
		\centering 
		\includegraphics[scale=0.9]{fig-G-to-Gp}
		\caption{The dashed ellipse represents the original graph $G$. One iteration adds all vertices and edges shown outside to. For simplicity, we label a vertex by its subscript.}
		\label{fig:G-to-Gp}
	\end{figure}
	
	We will present an elimination order of the constraints, so that $T'$ has the following desired structure: 
	\begin{enumerate}
		\item $p_T(v_i)$ is an ancestor of $v_i$ in $T'$ for all $i \in \{1,\dots,d\}$,
		\item $v_{\{i\}}$ is the parent of $v_i$ for all $i \in \{1,\dots,d\}$,
		\item for all triples of vertices $v_S, v_T, v_{S\cup T}$, where $S,T \subseteq [d]$, we have that $v_{S \cup T}$ is the parent of $v_S$ and $v_T$,
		\item for a vertex $v_S$ with $S \subseteq [d]$, if there does not exist another vertex $v_R$ such that $R \supset S$, then the parent of $v_S$ is $p_T(v_i)$ for any $i \in S$.
	\end{enumerate}

	Intuitively, a vertex $v$ with $k$ children in $T$ is transformed into a vertex $v$ at the root of a balanced binary tree with $k$ leaves in $T'$. Below is an illustration:
	 
	\begin{figure}[H]
		\centering 
		\includegraphics[scale=0.9]{fig-Tp}
		\caption{The elimination tree $T'$ locally at the vertex $v_8$. Inside the dashed box are the changes compared to $T$, caused by the new constraints from the current iteration. For simplicity, vertices are labelled by the subscripts in their names.}
		\label{fig:expanded-Tp}
	\end{figure}
	
	If we can produce the elimination tree described above, then it is straightforward to see that $height(T') \leq O(height(T) \cdot \log d)$, since at every level of $T$, our construction expands the height by a factor of at most $\log d$. Moreover, let $P(v_i)$ be the vertices between $v_i$ and $p_T(v_i)$ in $T'$. Then, if $t_i$ is the height of vertex $v_i$ in $T$ and $t'_v$ is the height of vertex $v$ in $T'$, we have
	\begin{align*}
		\sum_{v \in V(T')} t_v'^2 &= \sum_{i \in \{1,\dots, d\}} \left( t_{v_i}'^2 + \sum_{S \in P(v_i)} t_{v_S}'^2 \right) \\ 
		&\leq \sum_{i \in \{1,\dots,d\}} (t_i \log d)^2 + \log d \cdot (t_i \log d)^2 \\
		&\leq \log^4 d \cdot \sum_{i \in \{1,\dots,d\}} t_i^2.
	\end{align*}
	Hence, part (3) of the theorem statement would be satisfied.
	
	\subsection{Updated Elimination Order}
	Finally we present the elimination order for $G'$ that yields the elimination tree $T'$ as discussed above. 
	
	Without loss of generality, we may assume the elimination order for $G$ is the sequence $v_1, \dots, v_d$. 
	We will insert the remaining vertices into this sequence to arrive at the final ordering for $G'$. The rules are as follows:
	
	\begin{enumerate}
		\item vertex $v_{\{i\}}$ is eliminated immediately after vertex $v_i$ for each $i \in [d]$, and
		\item for any three vertices $v_S, v_T$, and $v_{S \cup T}$, where $S,T \subseteq [d]$, vertex $v_{S \cup T}$ is eliminated immediately after the latter of $v_S$ and $v_T$.
	\end{enumerate}

	As an example, suppose $G$ has eight vertices $\{v_1,\dots,v_8\}$, and its elimination tree $T$ is as shown Figure~\ref{fig:ex-elim-tree-old}. Then the ordering for $G'$ would be 
	\[
		v_1, v_{\{1\}}, v_2, v_{\{2\}}, v_{\{1,2\}}, v_3, v_{\{3\}}, v_4, v_{\{4\}}, v_{\{3,4\}}, v_{\{1,2,3,4\}}, v_5, v_{\{5\}}, v_6, v_{\{6\}}, v_{\{5,6\}}, v_7, v_{\{7\}}, v_{\{5,6,7\}}, v_8,
	\]
	which can be verified to generate $T'$ as shown in Figure~\ref{fig:expanded-Tp}.
	
	%More generally, for any $v_i \in V(T)$ with children $v_{j}, v_{j+1}, \dots, v_{j+k}$, the ordering of $V(G)$ has the form
	%\[
	%\dots, v_{j}, v_{j+1}, \dots, v_{j+k}, w, \dots, v_i, \dots
	%\]
	%where the $k$ children are consecutive in the ordering, and $w$ is some arbitrary vertex following $v_{j+k}$. New vertices of the form $v_S$ for $S \subseteq \{j, j+1, \dots, j+k\}$ introduced in iteration $v_i$ of Algorithm~\ref{alg:dense-col-mod} are inserted between $v_j$ and $w$ in the ordering for $G$.
	
	We prove a series of claims to show the correctness of the elimination order in producing the desired elimination tree. 
	
	For simplicity, we introduce some additional terminology: Given two vertices $u,v \in V(G)$ (resp. $G'$) with $u$ eliminated before $v$, we call a path $P$ from $u$ to $v$ an \emph{ancestor-certifying path} if all internal vertices on $P$ are eliminated before $u$. The existence of such a path implies that $v$ is an ancestor of $u$ in the elimination tree $T$ (resp. $T'$). 
	
	Given a vertex $v_S$ with $S \subseteq [d]$, since $p_T(v_i) = p_T(v_j)$ for any $i,j \in S$ by construction, we denote this unique vertex by $p_T(S)$. We also use $C(S)$ to denote the subtree in $G'$ with root $v_S$ and leaves $\{ v_i \;:\; i \in S\}$.
	
	Finally, let $\pi : V(G') \mapsto [|V(G')|]$ be the order on the vertices. 
	
	\begin{claim}
		The parent of vertex $v_i$ in $T'$ is $v_{\{i\}}$.
	\end{claim}
	\begin{proof}
	Since $v_iv_{\{i\}} \in E(G')$, this edge is an ancestor-certifying path from $v_i$ to $v_{\{i\}}$ in $G'$. 
	%Since $v_{\{i\}}$ is eliminated immediately after $v_i$, (i.e.
	Since $\pi(v_{\{i\}}) = \pi(v_i)+1$ (i.e. $v_{\{i\}}$ is eliminated immediately after $v_i$), the claim follows by the definition of parent.
	\end{proof}

	\begin{claim}\label{claim:who-is-parent}
		For any pair of vertices $v_S, v_R$, where $S \subset R \subseteq [d]$ and $R$ is the smallest subset containing $S$, $v_{R}$ is the parent of $v_S$ in $T'$.
	\end{claim}
	\begin{proof}
		Since $v_S v_{R}$ is an edge, it is also an ancestor-certifying path from $v_S$ to $v_{S \cup R}$. Suppose for a contradiction that $v \neq v_{R}$ is the vertex eliminated earliest after $v_S$ with an ancestor-certifying path from $v_S$ to it, implying $v$ is the parent of $v_S$ rather than $v_{R}$. 
		
		%Let $P$ be an ancestor-certifying path from $v_S$ to $v$. We claim that $v$ must be $v_k$ for some $k \in [d]$. 
		%Indeed, if $v = v_{U}$ for some $U \subseteq [d]$ with $|U| > 1$, then the second last vertex on $P$ must be $v_{U'}$ with $U' \subset U$, since other neighbours of $v_{U}$ are eliminated later.  guh $v_{S''}$ not necessarily right before $v_{S'}$.
		%However, $\pi(v_{S''}) = \pi(v_{S'}) - 1 > \pi(v_S)$, contradicting the fact that $P$ is an ancestor-certifying path from $v_S$ to $v_{S'}$. 
		%Alternatively, if $v$ were $v_{\{k\}}$ for some $k \in [d]$, then the second last vertex on $P$ must be $v_{U}$ for some $U \subseteq [d]$, such that $p_T(U) = v_k$. For any $i \in U$, we have $p_T(v_i) = v_k$, so there is an ancestor-certifying path from $v_i$ to $v_k$ in $G$ and therefore $G'$; denote this path by $Q$. Also, let $P'$ be the subpath of $P$ from $v_S$ to $v_U$; and let $P''$ be the path in $C(U)$ from $v_{U}$ to $v_i$. Note that for each vertex $w \in P''$, we have $\pi(v_i) \leq \pi(w) \leq \pi(v_{U}) < \pi(v_S)$, and for each vertex $w \in Q$, we have $\pi(w) < \pi(v_i)$. Hence $P' \cup P'' \cup Q$ is an ancestor-certifying path from $v_S$ to $v_k$, and $\pi(v_k) < \pi(v_{\{k\}})$, a contradiction.
		
		We can modify $P$ as follows: For every edge $v_U v_{\{j\}} \in P$, where $U \subseteq [d]$, $j \in [d]$, and $p_T(U) = v_j$, we can replace it by a path $P^+$, such that the resulting path is still ancestor-certifying from $v_S$ to $v_k$: Let $i \in U$, so $p_T(v_i) = v_j$. Let $Q$ be a ancestor-certifying path from $v_i$ to $v_j$ in $G$ and therefore $G'$, and let $Q'$ be the path from $v_i$ to $v_U$ in $C(U)$. All internal vertices $w$ on $Q$ satisfies $\pi(w) < \pi(v_i) < \pi(v_j)$, and all vertices $w$ on $Q'$ satisfies $\pi(w) < \pi(v_U) < \pi(v_j)$. Hence, $P^+ = Q' \cup Q \cup v_j v_{\{j\}}$ is a path from $v_U$ to $v_{\{j\}}$ that we use to replace the $v_U v_{\{j\}}$ in $P$. Similarly, we can replace edges $v_U v_j \in P$, where $U \subseteq [d], j \in [d]$, and $p_T(U) = v_j$. 
		
		\begin{figure}[H]
			\centering 
			\includegraphics[scale=0.9]{fig-edge-replacement}
			\caption{Recall the example of $G'$ locally, where $v_1, \dots, v_7$ are children of $v_8$ in $G$. A red edge in an ancestor-certifying path can be replaced by a path like the one in green labelled $Q \cup Q'$.}
		\end{figure}
		
		After this modification, $P$ is a union of 
		\begin{enumerate}
			\item A path $Q_1$ in $C(S)$ from $v_S$ to some $i \in S$,
			\item Type 1 paths, which are single edges of the form $v_a v_b$, where $a,b \in [d]$
			\item Type 2 paths, which are of the form $v_a, P', v_b$, where $a,b \in [d]$ and $p_T(a) = p_T(b)$, and $P' \subset C(S_{ab})$, where $S_{ab}$ is the set of smallest cardinality containing $a$ and $b$ such that $v_{S_{ab}} \in V(G')$
			\item If $v = v_U$ for some $U \subseteq [d]$, a path $Q_2$ in $C(U)$ from some $j \in U$ to $v_U$. Alternatively, if $v = v_k$ for some $k \in [d]$, we let $Q_2$ be the path with a single vertex $v_k$.
		\end{enumerate}
		
		Furthermore, without loss of generality, we may assume $v_i$ is the unique vertex on $P$ with $i \in S$, for otherwise we could shortcut $P$ while maintaining all the desired properties. Similarly, in the case that $v = v_U$, we may assume $v_j$ is the unique vertex on $P$ with $j \in U$. So we can write $P$ as $Q_1 \cup P' \cup Q_2$, where $P'$ is a union of type 1 and type 2 paths. We can view $P'$ as a directed path, and consider what happens as we traverse along it:
		
		Traversing along a Type 1 path $(v_a,v_b)$ can be viewed as moving from vertex $v_a$ to $v_b$ in $T$, where $v_b$ is an ancestor of $v_a$ if $a < b$, and vice versa. Traversing along a Type 2 path $(v_a, P', v_b)$ can be viewed as moving from vertex $v_a$ to $v_b$ in $T$, where $v_a$ and $v_b$ are children of the same parent.
		
		We begin with $v_i$ and traverse along $P'$ while making the corresponding moves in $T$ as described above. Note that all \emph{internal} vertices $v_l \in P$ that we move to must satisfy $\pi(v_l) \leq \pi(v_i)$. %, $\leq \pi(v_{\max S})$ is obvious, also only one $i \in S$ on $P$ is allowed. otherwise $P$ would not be an ancestor-certifying path from $v_S$ to $v$. %a few more words here
		It follows that all internal vertices on $P'$ we move to are contained in $T$ in the subtree rooted at $v_i$. If the final vertex on $P$ is $v = v_k$ for some $k \in [d]$, then we must have $i < k < j$, where $v_j = p_T(v_i)$, because of our initial assumption for a contradiction. However, in the last valid move in $T$, it is not possible to go from a vertex strictly in the subtree rooted at $v_i$ to such a vertex $v_k$. Alternatively, suppose the final vertex on $P$ is $v = v_U$ for some $U \subseteq [d]$. Let $v_j$ be the unique vertex on $P$ with $j \in U$. Then $v_j$ is an internal vertex on $P$ and therefore a descendant of $v_i$. It follows that $v_U$ must have been eliminated before $v_i$ by construction. Hence we get the desired contradiction.
	\end{proof}

	\begin{claim}
		For a vertex $v_S$ with $S \subseteq [d]$, if there does not exist $v_R$ with $R \supset S$, then the parent of $v_S$ in $T'$ is $p_T(S)$.
	\end{claim}
	\begin{proof}
		Suppose $v_p = p_T(S)$. Take arbitrarily $i \in S$, and note $v_p = p_T(v_i)$. %Note that if there does not exist $v_R$ with $R \supset S$, then $v_S$ is connected to $v_{\{j\}}$.	
		We know there is an ancestor-certifying path $P_T$ from $v_i$ to $v_p$ in $G$; since $G \subset G'$, there is the same ancestor certifying path $P_{T'}$ from $v_i$ to $v_p$ in $G'$. Furthermore, there is a path $Q$ from $v_S$ to $v_i$ in $C(S)$, and all vertices on this path are eliminated before $v_S$ by construction. Hence $Q \cup P_{T'}$ is an ancestor-certifying path from $v_S$ to $v_p$. 
		
		To see that there does not exist a vertex eliminated before $v_p$ with an ancestor-certifying path from $v_S$, we use a similar argument as in Claim~\ref{claim:who-is-parent}; the details are omitted.
	\end{proof}
\end{proof}
\end{comment}

